A Smoother Way to Train Structured Prediction Models

We present a framework to train a structured prediction model by performing smoothing on the inference algorithm it builds upon. Smoothing overcomes the non-smoothness inherent to the maximum margin structured prediction objective, and paves the way for the use of fast primal gradient-based optimization algorithms. We illustrate the proposed framework by developing a novel primal incremental optimization algorithm for the structural support vector machine. The proposed algorithm blends an extrapolation scheme for acceleration and an adaptive smoothing scheme and builds upon the stochastic variance-reduced gradient algorithm. We establish its worst-case global complexity bound and study several practical variants, including extensions to deep structured prediction. We present experimental results on two real-world problems, namely named entity recognition and visual object localization. The experimental results show that the proposed framework allows us to build upon efficient inference algorithms to develop large-scale optimization algorithms for structured prediction which can achieve competitive performance on the two real-world problems.

==> sections/table.tex <==
\begin{table*}[!thb]
\caption{{Smooth inference oracles for smoothed max margin training for structured prediction
with output $\yv = (y_1, \cdots, y_p)$ of size $p$.
This table shows how to obtain smooth inference oracles for various exact and approximate max oracles, 
$\ell_2$ and entropy smoothing. Here, $\mu$ is the level of smoothing and $\ell_2$ smoothing is computed using 
the top-$K$ largest entries.
For DP and graph cuts, $\mcT_{\max}$ denotes the running time of the max oracle.
% NAG stands for Nesteorv's accelerated gradient method~\citep{nesterov1983method}.
\vspace{2mm}
}}
\label{tab:rates}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ccc|cc|cc}

\toprule

\textbf{Max oracle} & \textbf{Cost} & \textbf{Exact?} & \multicolumn{2}{c}{\textbf{$\ell_2$ smoothing}} & 
	\multicolumn{2}{c}{\textbf{Entropy smoothing}} \\
 & & & Algo & Cost & Algo & Cost 
	\\ \hline\hline

\begin{tabular}{c} Dynamic Prog. \\ (Max Product) \end{tabular} & $\mcT_{\max}$ & Exact &
\begin{tabular}{c} Top-$K$ max prod \\ (algo.~\ref{algo:dp:topK:main}) \end{tabular}
	 & $\widetilde \bigO(K \mcT_{\max})$ &
\begin{tabular}{c} sum product \\ (algo.\ref{algo:dp:supp_exp}) \end{tabular} & $\bigO(\mcT_{\max})$ \\ \hline

Loopy BP &  & Approx. &
\begin{tabular}{c}  BMMF \\ (algo.~\ref{algo:top_k_map:general}) \end{tabular}
	 & \begin{tabular}{c} $\bigO(K)$ loopy \\ BP runs \end{tabular}  &
\multicolumn{2}{c}{Not possible} \\ \hline

\begin{tabular}{c} Graph cuts/ \\ matchings \end{tabular} & $\mcT_{\max}$ & Exact &
\begin{tabular}{c}  BMMF \\ (algo.~\ref{algo:top_k_map:general}) \end{tabular} &
\begin{tabular}{c}  $\bigO(pK \mcT_{\max})$ for cuts \\ $\bigO(K \mcT_{\max})$ for matchings \end{tabular}
	 &
\multicolumn{2}{c}{Not possible} \\ \hline

Search & ? & \begin{tabular}{c} Both \\ variants \end{tabular} & 
\begin{tabular}{c}  Top-$K$ search  \\ (algo.~\ref{algo:top_k:bb}) \end{tabular}
	& ? &
\multicolumn{2}{c}{Not possible} \\ \hline

% \begin{tabular}{c} LP \\ relaxation \end{tabular} & $\bigO(1/\eps)$ & $\eps$-approx &
% \begin{tabular}{c}  NAG \end{tabular} 
% 	& $\bigO(1/\sqrt{\mu \eps})$ &
% \begin{tabular}{c}  NAG \end{tabular} 
% 	& $\bigO(1/\sqrt{\mu \eps})$  \\ \hline

\bottomrule
\end{tabular}}
% \vspace{-1em}
\end{table*}


